Speed, Quality, and the Optimal Timing of Complex Decisions: Field Evidence

This paper presents an empirical investigation of the relation between decision speed and decision quality for a real-world setting of cognitively-demanding decisions in which the timing of decisions is endogenous: professional chess. Move-by-move data provide exceptionally detailed and precise information about decision times and decision quality, based on a comparison of actual decisions to a computational benchmark of best moves constructed using the artificial intelligence of a chess engine. The results reveal that faster decisions are associated with better performance. The findings are consistent with the predictions of procedural decision models like drift-diffusion-models in which decision makers sequentially acquire information about decision alternatives with uncertain valuations.

==> Results_Performance_Robust_FE_previous_moves.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{1.05\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{5}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{5}{c}{Best Move (Dummy)}                                                                        \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\emph{Decision Time}&                     &                     &                     &                     &                     \\
Time spent on move (min.)&     -0.0164\sym{***}&     -0.0164\sym{***}&     -0.0169\sym{***}&     -0.0170\sym{***}&     -0.0169\sym{***}\\
                    &    (0.0005)         &    (0.0005)         &    (0.0005)         &    (0.0005)         &    (0.0005)         \\
\emph{Complexity}   &                     &                     &                     &                     &                     \\
N Mega-nodes computed&     -0.0056\sym{***}&     -0.0056\sym{***}&     -0.0056\sym{***}&     -0.0056\sym{***}&     -0.0056\sym{***}\\
                    &    (0.0004)         &    (0.0004)         &    (0.0004)         &    (0.0004)         &    (0.0004)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     &                     \\
Distance second best move (log)&      0.1931\sym{***}&      0.1931\sym{***}&      0.1926\sym{***}&      0.1918\sym{***}&      0.1917\sym{***}\\
                    &    (0.0034)         &    (0.0034)         &    (0.0034)         &    (0.0034)         &    (0.0034)         \\
Remaining time (min.)&      0.0006\sym{***}&      0.0005\sym{**} &      0.0005\sym{**} &      0.0005\sym{**} &      0.0005\sym{**} \\
                    &    (0.0002)         &    (0.0002)         &    (0.0002)         &    (0.0002)         &    (0.0002)         \\
Time spent on move (previous own move)&                     &     -0.0013\sym{***}&     -0.0018\sym{***}&     -0.0013\sym{***}&     -0.0014\sym{***}\\
                    &                     &    (0.0004)         &    (0.0004)         &    (0.0004)         &    (0.0004)         \\
Time spent on move (previous opponent's move)&                     &                     &      0.0036\sym{***}&      0.0037\sym{***}&      0.0039\sym{***}\\
                    &                     &                     &    (0.0004)         &    (0.0004)         &    (0.0004)         \\
\emph{Decision Quality Previous Moves}&                     &                     &                     &                     &                     \\
Best move (previous own move)&                     &                     &                     &      0.0207\sym{***}&      0.0205\sym{***}\\
                    &                     &                     &                     &    (0.0035)         &    (0.0035)         \\
Best move (previous opponent's move)&                     &                     &                     &                     &      0.0076\sym{**} \\
                    &                     &                     &                     &                     &    (0.0037)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Number Move Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &       80359         &       80359         &       80359         &       80359         &       80359         \\
Game Observations   &        1592         &        1592         &        1592         &        1592         &        1592         \\
\bottomrule
\end{tabular*}
}


==> Results_Performance_baseline_FE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{0.9\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{6}{c}{Best Move (Dummy)}                                                                                              \\\cmidrule(lr){2-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\emph{Decision Time}&                     &                     &                     &                     &                     &                     \\
Time spent on move (min.)&     -0.0227\sym{***}&                     &                     &                     &     -0.0164\sym{***}&     -0.0189\sym{***}\\
                    &    (0.0006)         &                     &                     &                     &    (0.0005)         &    (0.0010)         \\
\emph{Time Budget}  &                     &                     &                     &                     &                     &                     \\
Remaining time (min.)&                     &     -0.0019\sym{***}&                     &                     &      0.0006\sym{***}&      0.0007\sym{***}\\
                    &                     &    (0.0002)         &                     &                     &    (0.0002)         &    (0.0002)         \\
\emph{Complexity}   &                     &                     &                     &                     &                     &                     \\
N Mega-nodes computed&                     &                     &     -0.0088\sym{***}&                     &     -0.0056\sym{***}&     -0.0050\sym{***}\\
                    &                     &                     &    (0.0005)         &                     &    (0.0004)         &    (0.0004)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     &                     &                     \\
Distance second best move (log)&                     &                     &                     &      0.2132\sym{***}&      0.1931\sym{***}&      0.1839\sym{***}\\
                    &                     &                     &                     &    (0.0036)         &    (0.0034)         &    (0.0035)         \\
\emph{Interactions} &                     &                     &                     &                     &                     &                     \\
Time spent X N Mega-nodes computed&                     &                     &                     &                     &                     &     -0.0002\sym{**} \\
                    &                     &                     &                     &                     &                     &    (0.0001)         \\
Time spent X Dist. second best move&                     &                     &                     &                     &                     &      0.0134\sym{***}\\
                    &                     &                     &                     &                     &                     &    (0.0020)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Number Move Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &       80359         &       80359         &       80359         &       80359         &       80359         &       80359         \\
Game Observations   &        1592         &        1592         &        1592         &        1592         &        1592         &        1592         \\
\bottomrule
\end{tabular*}
}


==> Results_Performance_baseline_FE_edited.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}cccccc}
\toprule
 &\multicolumn{6}{c}{Dependent Variable:}\\
                    &\multicolumn{6}{c}{Best Move (Dummy)}                                                                                              \\\cmidrule(lr){2-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\emph{Decision Time}&                     &                     &                     &                     &                     &                     \\
Time spent on move (min.)&     -0.0227\sym{***}&                     &                     &                     &     -0.0164\sym{***}&     -0.0189\sym{***}\\
                    &    (0.0006)         &                     &                     &                     &    (0.0005)         &    (0.0010)         \\
\emph{Time Budget}  &                     &                     &                     &                     &                     &                     \\
Remaining time (min.)&                     &     -0.0019\sym{***}&                     &                     &      0.0006\sym{***}&      0.0007\sym{***}\\
                    &                     &    (0.0002)         &                     &                     &    (0.0002)         &    (0.0002)         \\
\emph{Complexity}   &                     &                     &                     &                     &                     &                     \\
N Mega-nodes computed&                     &                     &     -0.0088\sym{***}&                     &     -0.0056\sym{***}&     -0.0050\sym{***}\\
                    &                     &                     &    (0.0005)         &                     &    (0.0004)         &    (0.0004)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     &                     &                     \\
Distance second best move (log)&                     &                     &                     &      0.2132\sym{***}&      0.1931\sym{***}&      0.1839\sym{***}\\
                    &                     &                     &                     &    (0.0036)         &    (0.0034)         &    (0.0035)         \\
\emph{Interactions} &                     &                     &                     &                     &                     &                     \\
Time spent $\times$ N Mega-nodes computed&                     &                     &                     &                     &                     &     -0.0002\sym{**} \\
                    &                     &                     &                     &                     &                     &    (0.0001)         \\
Time spent $\times$ Dist. second best move&                     &                     &                     &                     &                     &      0.0134\sym{***}\\
                    &                     &                     &                     &                     &                     &    (0.0020)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Number Move Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &       80359         &       80359         &       80359         &       80359         &       80359         &       80359         \\
Game Observations   &        1592         &        1592         &        1592         &        1592         &        1592         &        1592         \\
\bottomrule
\end{tabularx}
}


==> Results_Performance_intensive_margin_FE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{0.9\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{6}{c}{Move Quality (Log-Modulus)}                                                                                     \\\cmidrule(lr){2-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\emph{Decision Time}&                     &                     &                     &                     &                     &                     \\
Time spent on move (min.)&     -0.0091\sym{***}&                     &                     &                     &     -0.0103\sym{***}&     -0.0063\sym{***}\\
                    &    (0.0004)         &                     &                     &                     &    (0.0004)         &    (0.0008)         \\
\emph{Time Budget}  &                     &                     &                     &                     &                     &                     \\
Remaining time (min.)&                     &     -0.0001         &                     &                     &      0.0009\sym{***}&      0.0008\sym{***}\\
                    &                     &    (0.0002)         &                     &                     &    (0.0002)         &    (0.0002)         \\
\emph{Complexity}   &                     &                     &                     &                     &                     &                     \\
N Mega-nodes computed&                     &                     &     -0.0082\sym{***}&                     &     -0.0084\sym{***}&     -0.0089\sym{***}\\
                    &                     &                     &    (0.0006)         &                     &    (0.0006)         &    (0.0007)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     &                     &                     \\
Distance second best move (log)&                     &                     &                     &     -0.0259\sym{***}&     -0.0429\sym{***}&     -0.0307\sym{***}\\
                    &                     &                     &                     &    (0.0063)         &    (0.0065)         &    (0.0065)         \\
\emph{Interactions} &                     &                     &                     &                     &                     &                     \\
Time spent X N Mega-nodes computed&                     &                     &                     &                     &                     &      0.0002\sym{**} \\
                    &                     &                     &                     &                     &                     &    (0.0001)         \\
Time spent X Dist. second best move&                     &                     &                     &                     &                     &     -0.0174\sym{***}\\
                    &                     &                     &                     &                     &                     &    (0.0028)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Number Move Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &       80359         &       80359         &       80359         &       80359         &       80359         &       80359         \\
Game Observations   &        1592         &        1592         &        1592         &        1592         &        1592         &        1592         \\
\bottomrule
\end{tabular*}
}


==> Results_Performance_intensive_marging_FE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{1.05\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{6}{c}{Best Move (Dummy)}                                                                                              \\\cmidrule(lr){2-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\emph{Decision Time}&                     &                     &                     &                     &                     &                     \\
Time spent on move (min.)&     -0.0042         &                     &                     &                     &     -0.0706\sym{***}&      0.0199         \\
                    &    (0.0091)         &                     &                     &                     &    (0.0107)         &    (0.0313)         \\
\emph{Time Budget}  &                     &                     &                     &                     &                     &                     \\
Remaining time (hours)&                     &     -0.4727\sym{*}  &                     &                     &     -0.4165         &     -0.5363\sym{*}  \\
                    &                     &    (0.2833)         &                     &                     &    (0.2759)         &    (0.2776)         \\
\emph{Complexity}   &                     &                     &                     &                     &                     &                     \\
Seconds to reach fixed depth&                     &                     &      0.0170\sym{***}&                     &      0.0087\sym{***}&      0.0091\sym{**} \\
                    &                     &                     &    (0.0034)         &                     &    (0.0029)         &    (0.0041)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     &                     &                     \\
Distance second best move&                     &                     &                     &     -2.5120\sym{***}&     -2.5492\sym{***}&     -2.2850\sym{***}\\
                    &                     &                     &                     &    (0.2391)         &    (0.2424)         &    (0.2404)         \\
\emph{Interactions} &                     &                     &                     &                     &                     &                     \\
Seconds to reach fixed depth X Time spent&                     &                     &                     &                     &                     &      0.0036         \\
                    &                     &                     &                     &                     &                     &    (0.0034)         \\
Distance second best move X Time spent&                     &                     &                     &                     &                     &     -0.5050\sym{***}\\
                    &                     &                     &                     &                     &                     &    (0.1577)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Number Move Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &      105714         &      105714         &      105714         &      105714         &      105714         &      104105         \\
Game Observations   &        1973         &        1973         &        1973         &        1973         &        1973         &        1973         \\
\bottomrule
\end{tabular*}
}


==> Results_performance_robust_FE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{0.9\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{6}{c}{Best Move (Dummy)}                                                                                              \\\cmidrule(lr){2-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Time spent on move (min.)&     -0.0215\sym{***}&                     &                     &                     &     -0.0207\sym{***}&     -0.0222\sym{***}\\
                    &    (0.0006)         &                     &                     &                     &    (0.0006)         &    (0.0024)         \\
\emph{Time Budget}  &                     &                     &                     &                     &                     &                     \\
Time pressure phase before move 40&                     &     -0.0096\sym{*}  &                     &                     &     -0.0432\sym{***}&     -0.0430\sym{***}\\
                    &                     &    (0.0051)         &                     &                     &    (0.0051)         &    (0.0050)         \\
\emph{Complexity}   &                     &                     &                     &                     &                     &                     \\
N moves possible    &                     &                     &     -0.0057\sym{***}&                     &     -0.0036\sym{***}&     -0.0037\sym{***}\\
                    &                     &                     &    (0.0002)         &                     &    (0.0002)         &    (0.0003)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     &                     &                     \\
Standard deviation evaluation 6 best moves&                     &                     &                     &      0.0023\sym{***}&      0.0017\sym{***}&      0.0017\sym{***}\\
                    &                     &                     &                     &    (0.0001)         &    (0.0001)         &    (0.0001)         \\
\emph{Interactions} &                     &                     &                     &                     &                     &                     \\
N possible moves X Time spent&                     &                     &                     &                     &                     &      0.0000         \\
                    &                     &                     &                     &                     &                     &    (0.0001)         \\
Standard deviation evaluation X Time spent&                     &                     &                     &                     &                     &     -0.0000         \\
                    &                     &                     &                     &                     &                     &    (0.0000)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Move Number &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &       80359         &       80359         &       80359         &       80359         &       80359         &       80359         \\
Game Observations   &        1592         &        1592         &        1592         &        1592         &        1592         &        1592         \\
\bottomrule
\end{tabular*}
}


==> Results_time_taken_baseline_FE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{1\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{4}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{4}{c}{Time Spent on Move (minutes)}                                       \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
\emph{Time Budget}  &                     &                     &                     &                     \\
Remaining time (min.)&      0.0985\sym{***}&                     &                     &      0.0947\sym{***}\\
                    &    (0.0032)         &                     &                     &    (0.0032)         \\
\emph{Complexity}   &                     &                     &                     &                     \\
N Mega-nodes computed&                     &      0.0336\sym{***}&                     &      0.0193\sym{***}\\
                    &                     &    (0.0031)         &                     &    (0.0028)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     \\
Distance second best move (log)&                     &                     &     -0.9195\sym{***}&     -0.8294\sym{***}\\
                    &                     &                     &    (0.0241)         &    (0.0233)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         \\
Number Move Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &       80359         &       80359         &       80359         &       80359         \\
Game Observations   &        1592         &        1592         &        1592         &        1592         \\
\bottomrule
\end{tabular*}
}


==> Results_time_taken_baseline_FE_edited_text.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
%\begin{tabular*}{1\hsize}{@{\hskip\tabcolsep\extracolsep{-10pt}}l*{4}{D{.}{.}{-1}}}
\begin{tabularx}{0.75\textwidth}{l@{}cccc}
\toprule
 &\multicolumn{4}{c}{Dependent Variable:}\\
                    &\multicolumn{4}{c}{Time Spent on Move (minutes)}                                       \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
\emph{Time Budget}  &                     &                     &                     &                     \\
Remaining time (hours)&      5.6260\sym{***}&                     &                     &      5.5434\sym{***}\\
                    &    (0.1400)         &                     &                     &    (0.1402)         \\
\emph{Complexity}   &                     &                     &                     &                     \\
Seconds to reach fixed depth&                     &      0.0099\sym{***}&                     &      0.0080\sym{***}\\
                    &                     &    (0.0009)         &                     &    (0.0009)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     \\
Distance second best move&                     &                     &     -0.6956\sym{***}&     -0.6390\sym{***}\\
                    &                     &                     &    (0.0197)         &    (0.0183)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         \\
Number Move Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &      105714         &      105714         &      105714         &      105714         \\
Game Observations   &        1973         &        1973         &        1973         &        1973         \\
\bottomrule
%\end{tabular*}
\end{tabularx}
}


==> Results_time_taken_robust_FE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{1\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{4}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{4}{c}{Time spent on move (minutes)}                                       \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
\emph{Time Budget}  &                     &                     &                     &                     \\
Time pressure phase before move 40&     -1.3256\sym{***}&                     &                     &     -1.2581\sym{***}\\
                    &    (0.0411)         &                     &                     &    (0.0411)         \\
\emph{Complexity}   &                     &                     &                     &                     \\
N moves possible    &                     &      0.0541\sym{***}&                     &      0.0443\sym{***}\\
                    &                     &    (0.0021)         &                     &    (0.0021)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     \\
Standard deviation evaluation 6 best moves&                     &                     &     -0.0122\sym{***}&     -0.0080\sym{***}\\
                    &                     &                     &    (0.0006)         &    (0.0005)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         \\
Control Move Number &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &       80359         &       80359         &       80359         &       80359         \\
Game Observations   &        1592         &        1592         &        1592         &        1592         \\
\bottomrule
\end{tabular*}
}


==> Results_time_taken_robust_FE_edited_by_hand.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabularx}{\textwidth}{l@{\extracolsep{\fill}}ccccc}
\toprule
 &\multicolumn{4}{c}{Dependent Variable:}\\
                    &\multicolumn{4}{c}{Time spent on move (minutes)}                                       \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
\emph{Time Budget}  &                     &                     &                     &                     \\
Time pressure phase before move 40&     -1.3256\sym{***}&                     &                     &     -1.2581\sym{***}\\
                    &    (0.0411)         &                     &                     &    (0.0411)         \\
\emph{Complexity}   &                     &                     &                     &                     \\
N moves possible    &                     &      0.0541\sym{***}&                     &      0.0443\sym{***}\\
                    &                     &    (0.0021)         &                     &    (0.0021)         \\
\emph{Evaluation Gap}   &                     &                     &                     &                     \\                  
Standard deviation evaluation 6 best moves&                     &                     &     -0.0122\sym{***}&     -0.0080\sym{***}\\
                    &                     &                     &    (0.0006)         &    (0.0005)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         \\
Control Move Number &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &       80359         &       80359         &       80359         &       80359         \\
Game Observations   &        1592         &        1592         &        1592         &        1592         \\
\bottomrule
\end{tabularx}
}


==> Results_time_taken_robust_FE_previous_moves.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{1\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{5}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{5}{c}{Time Spent on Move (minutes)}                                                             \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\emph{Time Budget}  &                     &                     &                     &                     &                     \\
Remaining time (min.)&      0.0947\sym{***}&      0.0951\sym{***}&      0.0929\sym{***}&      0.0929\sym{***}&      0.0926\sym{***}\\
                    &    (0.0032)         &    (0.0032)         &    (0.0031)         &    (0.0031)         &    (0.0031)         \\
\emph{Complexity}   &                     &                     &                     &                     &                     \\
N Mega-nodes computed&      0.0193\sym{***}&      0.0193\sym{***}&      0.0197\sym{***}&      0.0199\sym{***}&      0.0199\sym{***}\\
                    &    (0.0028)         &    (0.0028)         &    (0.0026)         &    (0.0026)         &    (0.0026)         \\
\emph{Evaluation Gap}&                     &                     &                     &                     &                     \\
Distance second best move (log)&     -0.8294\sym{***}&     -0.8291\sym{***}&     -0.8286\sym{***}&     -0.8332\sym{***}&     -0.8296\sym{***}\\
                    &    (0.0233)         &    (0.0232)         &    (0.0228)         &    (0.0228)         &    (0.0227)         \\
\emph{Decision Time Previous Moves}&                     &                     &                     &                     &                     \\
Time spent on move (previous own move)&                     &      0.0053         &     -0.0125\sym{**} &     -0.0098\sym{**} &     -0.0087\sym{*}  \\
                    &                     &    (0.0049)         &    (0.0049)         &    (0.0050)         &    (0.0050)         \\
Time spent on move (previous opponent's move)&                     &                     &      0.1313\sym{***}&      0.1321\sym{***}&      0.1264\sym{***}\\
                    &                     &                     &    (0.0074)         &    (0.0074)         &    (0.0075)         \\
\emph{Decision Quality Previous Moves}&                     &                     &                     &                     &                     \\
Best move (previous own move)&                     &                     &                     &      0.1217\sym{***}&      0.1289\sym{***}\\
                    &                     &                     &                     &    (0.0292)         &    (0.0291)         \\
Best move (previous opponent's move)&                     &                     &                     &                     &     -0.2496\sym{***}\\
                    &                     &                     &                     &                     &    (0.0309)         \\
\midrule
Player-Game Fixed Effects&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Move Number &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Control Evaluation Position&         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Move Observations   &       80359         &       80359         &       80359         &       80359         &       80359         \\
Game Observations   &        1592         &        1592         &        1592         &        1592         &        1592         \\
\bottomrule
\end{tabular*}
}


==> Summary_per_game.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccccc}}
\toprule
                    &       Games&        Mean&   Std. Dev.&         Min&         Max\\
\midrule
\emph{Player strength}&            &            &            &            &            \\
Elo rating white player&       1,982&      2681.7&       85.24&        2500&        2881\\
Elo rating black player&       1,982&      2681.0&       85.09&        2500&        2881\\
\emph{Game result}  &            &            &            &            &            \\
White player wins   &       1,982&       0.279&       0.448&           0&           1\\
Draw                &       1,982&       0.566&       0.496&           0&           1\\
Black player wins   &       1,982&       0.156&       0.363&           0&           1\\
\emph{Duration}     &            &            &            &            &            \\
Num. moves overall  &       1,982&       41.04&       14.55&          15&          98\\
Duration game (hours) overall&       1,982&       3.332&       1.443&           0&       8.113\\
\bottomrule
\end{tabular}
}


==> Summary_stats_baseline.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccccc}}
\toprule
                    &       Moves&        Mean&   Std. Dev.&         Min&         Max\\
\midrule
\emph{Decision Quality}&            &            &            &            &            \\
Best move (dummy)   &     105,733&       0.623&       0.485&           0&           1\\
Move quality (log-modulus)&     105,733&      -0.125&       0.381&      -6.485&       5.602\\
\emph{Decision Time}&            &            &            &            &            \\
Time spent on move (min.)&     105,733&       2.497&       4.080&           0&       100.5\\
\emph{Time Budget}  &            &            &            &            &            \\
Remaining time (hours)&     105,733&       0.665&       0.528&           0&       2.513\\
Time pressure phase before move 40&     105,733&       0.238&       0.426&           0&           1\\
\emph{Complexity}   &            &            &            &            &            \\
Seconds to reach fixed depth&     105,733&       30.50&       24.12&     0.00200&       799.3\\
Best move restricted engine (dummy)&     105,733&       0.660&       0.474&           0&           1\\
\emph{Evaluation Gap}&            &            &            &            &            \\
Distance second best move&     105,733&       0.420&       0.796&           0&       6.485\\
Standard deviation evaluation 6 best moves&     105,733&       6.734&       29.97&           0&       327.0\\
\bottomrule
\end{tabular}
}

